Reinforcement Learning with Almost Sure Constraints

In this work we address the problem of finding feasible policies for Constrained Markov Decision Processes under probability one constraints. We argue that stationary policies are not sufficient for solving this problem, and that a rich class of policies can be found by endowing the controller with a scalar quantity, so called budget, that tracks how close the agent is to violating the constraint. We show that the minimal budget required to act safely can be obtained as the smallest fixed point of a Bellman-like operator, for which we analyze its convergence properties. We also show how to learn this quantity when the true kernel of the Markov decision process is not known, while providing sample-complexity bounds. The utility of knowing this minimal budget relies in that it can aid in the search of optimal or near-optimal policies by shrinking down the region of the state space the agent must navigate. Simulations illustrate the different nature of probability one constraints against the typically used constraints in expectation.

==> equivalence.tex <==
\subsection{Are $Q(s,a)$ and $k_\star(s,a)$ enough?}

Define $\mathcal A^\star(s,k)=\{a\in\mathcal A:\ B_\star(s,k,a)=0\}=\{a\in\mathcal A:\ k_\star(s,a) \leq k\}$

Algorithm 1 (Uses previously learned $\mathcal A(s,k)$)

$$Q^{t+1}(s_t,a_t)= Q^{t}(s_t,a_t)+\alpha_t\left(r(s_t,a_t)+\max_{a'\in\mathcal A(s_{t+1},k_{t+1})}Q^t(s_{t+1},a') -Q(s_t,a_t)\right)$$

defining  $\max_{a'\in\mathcal A(s_{t+1},k_{t+1})}Q^t(s_{t+1},a')=-\infty$ when $\mathcal A(s_{t+1},k_{t+1})=\emptyset$  

Algorithm 2 (Standard Q-learning for the augmented state)

$$\bar Q^{t+1}(s_t,k_t,a_t)=\bar Q^{t}(s_t,,k_t,a_t)+\alpha_t\left(r(s_t,k_t,a_t)+\max_{a'\in\mathcal A}\bar Q^t(s_{t+1},k_{t+1},a')-\bar Q(s_t,k_t,a_t) \right)$$


Claim: $$\bar Q^\infty(s,k,a)=\begin{cases}-\infty &\ if\ k<k_\star(s,a)\\
Q^{\infty}(s,a)&\ otherwise\end{cases}$$

Proof (incomplete)
$Q^\infty(s,k,a)=Q_\star(s,k,a)=-\infty$ if $k<k_\star(s,a)$\\

It remains to proof that $\bar Q^\infty(s,k,a)=
Q^{\infty}(s,a)$   when $k\geq k_\star(s,a)$

Knowing the limit of Algorithm 2, we can modify it in order to avoid futile  iterations whenever we have the triplets $(s_t,k_t,a_t)$ such that  $Q_\star(s_t,k_t,a_t)=-\infty$. More specifically, when $k_t<k_\star(s_t,a_t)$ $Q_\star(s_t,k_t,a_t)=-\infty$, and 

$$\max_{a'\in\mathcal A}\bar Q_\star(s_{t+1},k_{t+1},a')=\max_{a'\in\mathcal A_\star(s_{t+1},k_{t+1})}\bar Q_\star(s_{t+1},k_{t+1},a')$$

Hence (not entirely sure about this hence, may need a proof) Algorithm 2 converges to the same limit as Algorithm 3.

$$\tilde Q^{t+1}(s_t,k_t,a_t)=\begin{cases}&-\infty \ if\ k_t<k_\star(s_t,a_t)\\
&\tilde Q^{t}(s_t,k_t,a_t)+\alpha_t\left(r(s_t,a_t)+\max_{a'\in\mathcal A_\star(s_{t+1},k_{t+1})}\tilde Q^t(s_{t+1},k_{t+1},a')-\tilde Q(s_t,k_t,a_t) \right)\end{cases}$$

It remains to proof that we can remove $k_t$ from $\tilde Q(s_t,k_t,a_t)$ because $k_t$ is already accounted for when maximizing over when $A_\star(s_{t+1},k_{t+1})$ (not entirely sure if that is true)

\clearpage
\section*{Algorithm graveyard}
\begin{algorithm}
\caption{Online minimal budget learner}
\KwResult{$k^*(s,a)~\forall (s,a)$}
Initialize $k(\cdot,\cdot)=0$\;

\For{$t=0,1,\cdots$}{
    Sample $(S_t,A_t)\sim \operatorname{Unif}(\mathcal{S}\times\mathcal{A})$\\
    \eIf{$k(S_t,A_t)>\Delta$}{
      \tcc{State-action pair is unsafe, resample.}
      \textbf{continue}
    }{Sample $(S_t',D_t')$ transition.
    
    \tcc{Update minimal budget}
      $k(S_t,A_t)\leftarrow\max\left\{k(S_t,A_t); D_{t}'+\min_{a'}k(S_{t}',a')\right\}$
    }
}
\label{alg:online-budget-learner}
\end{algorithm}

\begin{algorithm}
\caption{Offline minimal budget learner}
\KwResult{$k^*(s,a)~\forall (s,a)$}
\tcc{Sampler}
\For{$(s,a)\in\mathcal{S}\times\mathcal{A}$}{
    Sample $N$ transitions $(s,a)\rightarrow(s',d)$
}
Build estimate kernel $\hat{\mathbb{P}}(s',d|s,a)=\frac{\operatorname{count}(s',d;s,a)}{N}$\;

Compute marginals $\hat{\mathbb{P}}(s'|s,a)\text{~and~}\hat{\mathbb{P}}(d=1|s,a,s')$

\tcc{Learner}
\For{$c=0,1,\ldots$}{
    \For{$(s,a)\in\mathcal{S}\times\mathcal{A}$}{
        $k(s,a) \leftarrow \max_{s':\hat{\mathbb{P}}(s'|s,a)>0}\left\{\mathds{1}\left(\hat{\mathbb{P}}(d=1|s,a,s')\right)+\min_{a'}k(s',a')\right\}$
    }
}
\label{alg:offline-budget-learner}
\end{algorithm}
\agustin{I'm thinking maybe we should go for Algo \ref{alg:offline-budget-learner} instead of \ref{alg:online-budget-learner}. Claim should be something like:\\
1) sample-complexity to get ``consistent'' kernel.
2) If consistent kernel $\rightarrow$ Algo \ref{alg:offline-budget-learner} converges to optimal $k^*~\forall (s,a) : k^*(s,a)\leq \Delta$ }


